Pyramid: Enhancing Selectivity in Big Data Protection with Count Featurization

Protecting vast quantities of data poses a daunting challenge for the growing number of organizations that collect, stockpile, and monetize it. The ability to distinguish data that is actually needed from data collected "just in case" would help these organizations to limit the latter's exposure to attack. A natural approach might be to monitor data use and retain only the working-set of in-use data in accessible storage; unused data can be evicted to a highly protected store. However, many of today's big data applications rely on machine learning (ML) workloads that are periodically retrained by accessing, and thus exposing to attack, the entire data store. Training set minimization methods, such as count featurization, are often used to limit the data needed to train ML workloads to improve performance or scalability. We present Pyramid, a limited-exposure data management system that builds upon count featurization to enhance data protection. As such, Pyramid uniquely introduces both the idea and proof-of-concept for leveraging training set minimization methods to instill rigor and selectivity into big data management. We integrated Pyramid into Spark Velox, a framework for ML-based targeting and personalization. We evaluate it on three applications and show that Pyramid approaches state-of-the-art models while training on less than 1% of the raw data.

==> Makefile <==
PAPER=paper
LATEX=pdflatex

BIBTEX=bibtex

DIFF=diff
DIFFHASH=1defb021d402be01d42b96ab211482edb6e37453
LATEXDIFF=latexdiff
DIFFDIR=diff2_tex

SRCS=$(wildcard *.tex)
REFS=$(wildcard *.bib)
FIGS=$(wildcard figures/*)

.PHONY: results $(PAPER).pdf clean diff diff_setup

all: $(PAPER).pdf

diff_setup:
	@echo "Automatic setup is not working yet."
	cat latexdiff_preamble.txt > $(DIFFDIR)/$(PAPER).tex.tmp
	cat $(DIFFDIR)/$(PAPER).tex >> $(DIFFDIR)/$(PAPER).tex.tmp
	mv $(DIFFDIR)/$(PAPER).tex.tmp $(DIFFDIR)/$(PAPER).tex
	#git clone git@github.com:columbia/pyramid-paper.git $(DIFFDIR) $(DIFFHASH)
	#cat latexdiff_preamble.txt > $(DIFFDIR)/$(PAPER).tex.tmp
	#cat $(DIFFDIR)/$(PAPER).tex >> $(DIFFDIR)/$(PAPER).tex.tmp
	#mv $(DIFFDIR)/$(PAPER).tex.tmp $(DIFFDIR)/$(PAPER).tex

diff:
	echo "% Required File" > latexdefs.tex
	echo "% Required File" > mathnotation.tex
	echo "% Required File" > $(DIFFDIR)/latexdefs.tex
	echo "% Required File" > $(DIFFDIR)/mathnotation.tex
	$(LATEXDIFF) --exclude-textcmd="section,subsection" --flatten $(DIFFDIR)/$(PAPER).tex $(PAPER).tex > $(DIFF).tex
	$(LATEX) $(DIFF)
	$(LATEX) $(DIFF)
	$(LATEX) $(DIFF)

results:
	+make -C $@

$(PAPER).pdf: $(SRCS) $(REFS) $(FIGS)
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)


submission: $(PAPER).pdf
	cp $(PAPER).pdf submission/

clean:
	rm -f *.dvi *.aux *.log *.blg *.bbl \
          $(PAPER).ps $(PAPER).pdf \
          $(PAPER)-single.pdf $(PAPER)-single.ps\
	  $(DIFF).pdf $(DIFF).tex


==> analysis.tex <==
\section{Security Analysis}
\label{sec:analysis}

- Repeat the protection properties (P1, P2, and P3 from
\S\ref{sec:threat-model} and stress the limitations.

- Talk about composability of \sysname with any number of other protection
options (i.e., make it clear that Pyramid doesn't get to decide the specific
protections applied to various kinds of stores).


==> conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}

